Recovery guarantee of weighted low-rank approximation via alternating minimization

Many applications require recovering a ground truth low-rank matrix from noisy observations of the entries, which in practice is typically formulated as a weighted low-rank approximation problem and solved by non-convex optimization heuristics such as alternating minimization. In this paper, we provide provable recovery guarantee of weighted low-rank via a simple alternating minimization algorithm. In particular, for a natural class of matrices and weights and without any assumption on the noise, we bound the spectral norm of the difference between the recovered matrix and the ground truth, by the spectral norm of the weighted noise plus an additive error that decreases exponentially with the number of rounds of alternating minimization, from either initialization by SVD or, more importantly, random initialization. These provide the first theoretical results for weighted low-rank via alternating minimization with non-binary deterministic weights, significantly generalizing those for matrix completion, the special case with binary weights, since our assumptions are similar or weaker than those made in existing works. Furthermore, this is achieved by a very simple algorithm that improves the vanilla alternating minimization with a simple clipping step. The key technical challenge is that under non-binary deterministic weights, na\"ive alternating steps will destroy the incoherence and spectral properties of the intermediate solutions, which are needed for making progress towards the ground truth. We show that the properties only need to hold in an average sense and can be achieved by the clipping step. We further provide an alternating algorithm that uses a whitening step that keeps the properties via SDP and Rademacher rounding and thus requires weaker assumptions. This technique can potentially be applied in some other applications and is of independent interest.

==> precise_statement.tex <==
%!TEX root = main.tex
\section{Precise statement of our result and comparison with prior work} \label{sec:precise_statement}

This section is an auxiliary section which will be removed in the final version, it contains: 

(1). Precise Statement of our result (quantitively) and all the parameters. 

(2). Precise Technical comparison with other works. 



REMEMBER: NO simplification has been made to those parameters, these are PRECISE relations we need. We need to put simplified relations to the final version. 

\subsection{Assumptions}

~

(1). Original matrix: $$\bMg  = \bU \bSigma \bV^{\top}$$

 where $\bU, \bV$ are $\mu - incoherent$ rank $k$ orthogonal matrices, $\sigma_{\max}(\bSigma) \le 1$. 

(2). Weighted matrix: $\bW$ such that $$||\bW - \bE||_2 \le \gamma n$$,

 where $\gamma < 1$, $\bE$ is the all one matrix. We have $\gamma n$ instead of $\gamma$ because $||\bE||_2 = n$. 

(3). Noise matrix: $\bNoise$ such that $$||\bW \hp \bNoise ||_2 \le \delta$$


(4). Correlation with ground truth: $\bD_i = \diag(\bW_i)$, for all $i \in [n]$

$$\lambdal \bI \preceq \bU^{\top} \bD_i \bU \preceq \lambdau \bI$$
$$\lambdal \bI \preceq \bV^{\top} \bD_i \bU \preceq \lambdau \bI$$



\subsection{Parameter relations}

(1).  This says $\lambdal$ is not too small. Note with our current scaling, typically $\lambdau, \lambdal = \Theta(1)$. $$\lambdal \ge \frac{32 k^2 \mu || \bW||_{\infty} \log n}{n} \lambdau$$

(2). This says $\gamma$ is small.  $$\gamma k\left( k \mu + \frac{12}{\lambdal^2}{\lambdau^2} \mu + \frac{3k \delta^2}{n \lambdal^2} \right) \le \frac{1}{2}$$


(3). This says $\gamma$ is small (actually this is strictly stronger than (2) if $\lambdau, \lambdal = \Theta(1)$). $$\frac{\gamma k \mu }{\sigma_{\min}(\bMg)} \times (16 k \sqrt{\log n}) \le \frac{1}{4}$$


In words, we need $\gamma < \frac{1}{k^2 \mu \sqrt{\log n}}$, $\delta < \frac{1}{k \sqrt{\log n}}$. 


\subsection{Our result}

After $t$ iterations, we will recover an matrix $\btM$ such that $||\btM - \bMg||_2 \le \frac{1}{2^t} + O(k \sqrt{\log n} ) \delta$. 

So we actually blow up the noise by $ O(k \sqrt{\log n} )$





\section{Technical comparison to other results}


NOTE: ALL the other noisy matrix completion papers mention that they DECREASE noise, but this is CHEATING, none of them actually decreases the noise. 

\subsection{Noisy matrix completion}

\subsubsection{Result comparision}


Their result is: given $\Omega$, $|\Omega| = pn^2 \ge n \mu^4 \log^2 n$ ($\mu$ is the incoherent parameter) as the indices of (random) observed entries, ground truth matrix $\bMg$ whose rank $k = O(1)$ and the noisy observation $\bM$ such that $|| \bMg - \bM||_{\Omega} \le \delta_1$ (which means $\sum_{(i, j) \in \Omega} ( \bMg - \bM)_{i, j}^2 \le \delta_1^2$). Their algorithm is

$$\min ||\btM||_{*} \quad s.t. ||\bM - \btM||_{\Omega} \le \delta$$

\Anote{Something fishy with the $\delta$ and $\delta_1$. Seems to me like the guarantee should just be $|| \bMg - \bM||_{\Omega} \le \delta$ and $\delta_1$ shouldn't appear. See section 2.}

Which recovers an matrix $\btM$ such that 
$$||\btM - \bM||_F \le 4 \sqrt{\frac{(2 + p) n}{p}}\delta_1 + 2 \delta_1$$




\Ynote{PLEASE CHECK CAREFULLY} Cast to our language: $\gamma = \sqrt{\frac{1}{pn}}$, $\delta = \frac{\delta_1}{\sqrt{p}}$. Therefore, their result is

$$||\btM - \bM||_F \le \sqrt{n} || \bNoise||_{F}$$

Therefore, 

(1). They blow up the noise by $\sqrt{n}$, which seems very bad. 

(2). Their argument doesn't contain the case when $k = \Omega(1)$ (I didn't find it in their paper).

(3). Their argument needs $\gamma \le \frac{1}{\mu^2 \log n}$, which seems worse than us. 

(4). Their argument is in $|| *||_F$, which is weaker than $||*||_2$. 

\subsubsection{Technique comparision}

~

The main problem is WHY, ON EARTH, our problem can NOT be solved using the simple SDP relaxation.

$$ \min ||\btM||_{*} \quad s.t. ||\bW \hp (\btM - \bM)||_2 \le \delta$$



From my point of view, this is because their proof needs to construct a dual certificate $\bLambda = \sP_{\Omega}(\bLambda)$ ($\sP_{\Omega}$ is the projection onto $\Omega$) such that 

(1). Let $\bT$ be the linear spam of columns of $\bU, \bV$, $\bTb$ be the orthogonal space, then 
$||\sP_{\bTb}(\bLambda)|| \le \frac{1}{2}$

(2). $\sP_{\bT} \sP_{\Omega} \sP_{\bT} \succeq \frac{p}{2} \bI$


However, if one just replace $\sP_{\Omega}$ operator by $\bW \hp$ operator, when the weight matrix is $\bW$ instead of $\Omega$, one can not hope to find $\bLambda$ such that $\bW \hp \bLambda = \bLambda$. Moreover, one does NOT have $\bW \hp \bW \hp \bA = \bW \hp \bA$, but $\sP_{\Omega}^2 = \sP_{\Omega}$ is necessary in their proof. 



Moreover, there is 



\subsection{Universal Matrix Completion}


\subsubsection{Result comparision}



Their result is: given $\Omega$, $|\Omega| = dn$ as the indices of observed entries, ground truth matrix $\bMg$, and 

(1). $\Omega$ is an expander graph: $\sigma_1(\Omega) = d$, $\sigma_2(\Omega) \le c \sqrt{d}$.

(2). $d \ge c^2 \mu^2 k^2$. 

Their algorithm:
$$\min ||\btM||_{*} \quad s.t. \sP_{\Omega}(\btM) = \sP_{\Omega}(\bM) $$


Which recovers the $\bM$ exactly.


 \Ynote{PLEASE CHECK CAREFULLY} Cast to our language: $\gamma = \sqrt{\frac{1}{d}} = \frac{1}{\mu k}$.
 
 
 Therefore, 
 
(1).  For the requirement on $\gamma$, it is weaker than us, so at this point they are better.  

(2). However, they need very strong expansion: $\sigma_2(\Omega) \le c \sqrt{d}$, which is worse than us.

(3). They only consider 0, 1 case, and the graph is $d$-regular. 

(4). They don't have tolerance of noise. 

\subsubsection{Technique comparision}

It doesn't work in our setting same as noisy matrix completion. 



\subsection{Matrix completion from noisy entries}

This is the Grassmann manifold paper. 


\subsubsection{Result comparision}

Their result is: given $\Omega$ random sampled entries from noisy matrix: $\bM = \bMg + \bNoise$, then they can recover $\btM$ such that  (you see it correctly, the noise is in spectral norm, $\bNoise_{\Omega}$ is the noise restricted on $\Omega$)
$$\frac{1}{n}  \leftll  \bMg - \btM \rightll_F = O \left(||\bMg||_{\infty} \left(\frac{n k}{|\Omega|} \right)^{1/2}  + \frac{n \sqrt{k}}{|\Omega|}||\bNoise_{\Omega}||_2\right)$$


They have another version of the theorem: For $|\Omega| \ge Cn \frac{\sigma_{\max}(\bMg)^2}{\sigma_{\min}(\bMg)^2} \mu k \log n$, 
$$\frac{1}{n}  \leftll  \bMg - \btM \rightll_F = O \left( \frac{n \sqrt{k}}{|\Omega|} \frac{\sigma_{\max}(\bMg)^2}{\sigma_{\min}(\bMg)^2}||\bNoise_{\Omega}||_2\right)$$



\Ynote{PLEASE CHECK CAREFULLY} Cast to our language: They actually have: $\gamma \ge \sqrt{\frac{1}{\mu k \log n}}$ with
$$||\bMg - \btM||_F = O(n \sqrt{k} ||\bNoise||_2)$$


Therefore

(1). The grantee is only on $||*||_F$, which is bad.

(2). Their requirement of $\gamma$ is weaker than ours, which is good.  

(3). They also blow up the noise. Note that $||\bMg - \btM||_2 \ge \frac{1}{n } ||\bMg - \btM||_F $

(4). Their algorithm is very inefficient. 


\subsubsection{Technique comparision}

Their algorithm doesn't work for our setting in an obvious way: their result heavily rely on the random sample, if $\Omega$ is random, then $\E[\bM_{\Omega}] \propto \bM$ for every $\bM$. However for our case it is far from being true. Moreover, their analysis is on $||*||_F$ because $\E[||\bM_{\Omega}||_F] \propto ||\bM||_F $ and their measurement of distance: $d(\bU, \bX) = \sqrt{ \trace(\bU^{\top} \bX \bX^{\top} \bU)}$ is proportional to $||\bU - \bX||_F$. All the analysis works in $||*||_F$ which does not extend to our $||*||_2$ result.


More precisely, their algorithm works in this way:

(1). The \emph{Gradient} of their objective function is somewhat proportional to $||\btM - \bM||_{\Omega}$, which is with high probability (due to random sample) close to $||\btM - \bM||_{F}$ which is $d(\bM, \btM)$. 

(2). Their algorithm is gradient descent, which reduces the gradient at each step. By (1), they actually reduce the distance. 


\subsection{Alternative Minimization}

This is the Moritz paper.




\subsubsection{Result comparision}


Given random sample $|\Omega| = pn^2$ entries, and $\bM = \bMg + \bNoise$, and $\bNoise$ satisfies the following constrains: (1). $\mu(\bNoise) \le \mu(\bMg) = \mu$, (2). $||\bNoise||_{\infty} \le \frac{\mu}{n} ||\bMg||_F$. Then their algorithm recovers $\btM$ such that $$||\btM - \bM||_F \le \varepsilon || \bM||_F$$

Provided that ($\sigma_k$ is the $k$-th singular value of rank $k$ matrix $\bMg$). $$pn \ge k (k + \log (n/\varepsilon)) \mu \times \left( \frac{||\bMg||_F + ||\bNoise||_F/\varepsilon}{\sigma_k}\right)^2 \left( 1 - \frac{||\bNoise||_2}{\sigma_k} \right)^5$$


\Ynote{PLEASE CHECK CAREFULLY} Cast to our language: They actually have: $\gamma = \frac{1}{k \sqrt{\mu  \log n}}$ with
$$||\btM - \bM||_F \le ||\bNoise||_F $$


Therefore,

(1). Their requirement of $\gamma$ is weaker than us, but not much.

(2). They doesn't blow up noise, however, they require noise matrix to be somewhat incoherent and has small entry-wise error, which is much more structured than ours. 


 \subsubsection{Technique comparision}
 
 Their technique is very similar to us as for the update analysis. In order for it to work they also has a whitening step, however, it is much weaker than us because their whitening is essentially a matrix concentration bound: As we will see, through out the analysis we need $\bX^{\top} \bD_i \bX$ ($\bD_i = \diag(\bW_i)$) to have large eigenvalues, however, in their random case this is very easy, since $\bX^{\top} \bX = \bI$ and $\E[\bD_i] = \bI$, therefore $\E[\bX^{\top} \bD_i \bX] = \bI$. What we need is just matrix concentration bound plus some median estimator (which has higher concentration than mean). Their whole argument breaks down in our case due to no randomness in the weight matrix. Therefore, our whitening step is much more involved.  
 
 



==> randominit.tex <==

\subsection{Random initialization} 

\begin{lem}\label{lem:sigma_init}
Let $\bY$ be a random matrix in $\mathbb{R}^{n \times k}$ generated as $\bY_{i,j} = b_{i,j} \frac{1}{\sqrt{n}}$, where $b_{i,j}$ are independent, uniform $\{-1,1\}$ variables.  

%$\mathcal{N}(0,\frac{1}{n})$ (independently), rejecting if $\exists j \in [n], \|\bY^j\|^2_2 \ge 10 \frac{k}{n}$. 
With probability $1-\frac{1}{\mbox{poly}}$ over the draw of $\bY$,  
$$\forall i, \sigma_{\min}\left(\bY^{\top} \bD_i \bY\right) \ge \frac{1}{4} \frac{\lambdal}{k \mu} $$ 
%$$\forall i, \sigma_{\max}\left(\bY^{\top} \bD_i \bY\right) \le \frac{5}{4} \frac{D_1}{n}  $$ 
 %$ \| \bY - \bV \|_2 \le \frac{\lambdal^2 n}{36 \mu k^2 \dmax}$, then 
%$$\left| \left\{ i  \in [n]\left| \sigma_{\min} (\bY^{\top} \bD_i \bY) \le \frac{\lambdal}{4} \right. \right\} \right| \le \frac{54 \mu^2 k^3 \gamma^2 \dmax}{\lambdal^2} \| \bV - \bY \|_2^2 $$
\end{lem}

\begin{proof}[Proof of Lemma \ref{lem:sigma_init}]

Notice that $\bY^{\top} \bD_i \bY  = \sum_j (\bY^j)^{\top} (\bD_i)_j \bY^j $, and each of the terms $(\bY^j)^{\top} (\bD_i)_j \bY^j$ is independent. 
Furthermore, it's easy to see that $\mathbb{E} [(\bY^j)^{\top} (\bD_i)_j (\bY^j)] = \frac{1}{n} (\bD_i)_j$, $\forall j$. %\yingyu{?} 
By linearity of expectation it follows that 
$\mathbb{E}[ \sum_j (\bY^j)^{\top} (\bD_i)_j \bY^j] = \frac{1}{n} \sum_j (\bD_i)_j $.

Now, we claim  $\sum_j (\bD_i)_j \ge \frac{\lambdau n}{k\mu}$. Indeed, by our assumption on $\bV$ we have for any vector $a \in \mathbb{R}^n$  
$$a^{\top} \bV^{\top} \bD_i \bV a = \sum_j (\bD_i)_j \langle \bV^j, a \rangle^2 \ge \lambdal $$
On the other hand however, by incoherency of $\bV$, $\sum_j (\bD_i)_j \langle \bV^j, a \rangle^2  \le \sum_j (\bD_i)_j \frac{\mu k}{n} $.  
Hence, $\sum_j (\bD_i)_j \ge \lambdau \frac{n}{k \mu}$. Putting things together, we get
$$\mathbb{E}[ \sum_j (\bY^j)^{\top} (\bD_i)_j \bY^j] \ge \frac{\lambdal}{k\mu}$$

Let's denote 
$$R := \|(\bY^j)^{\top} (\bD_i)_j \bY^j\|_2 \le \frac{k}{n} (\bD_i)_j \le \frac{\lambdal}{k \mu\log^2 n}$$ 
where the first inequality follows from our sampling procedure, and the last inequality by the assumption that $\|W\|_{\infty} \leq \frac{\lambdal n}{k^2 \mu \log^2 n}$. 

Since all the random variables $(\bY^j)^{\top} (\bD_i)_j \bY^j$ are independent, applying Matrix Chernoff we get that
$$ \Pr\left[ \sum_j (\bY^j)^{\top} (\bD_i)_j (\bY^j) \le (1-\delta) \frac{\lambdal}{k \mu}\right] \le n \left(\frac{e^{-\delta}}{(1-\delta)^{(1-\delta)}}\right)^{\frac{\lambdal}{k \mu R}} \le n \left(\frac{e^{-\delta}}{(1-\delta)^{(1-\delta)}}\right)^{\log^2 n} $$ 

Picking $\delta = \frac{3}{4}$, and union bounding over all $i$, with probability $1 - \frac{1}{\mbox{poly}}$, for all $i$,  
$$ \sigma_{\min}\left(\bY^{\top} \bD_i \bY\right)  \ge \frac{1}{4} \frac{\lambdal}{k \mu}$$
as we needed. 
%
%We proceed now to the upper bound on $\sigma_{\max}$, 
%By our assumption, $\sum_j (\bD_i)_j \le D_1$. Hence, $\mathbb{E}\left[ \sum_j (\bY^j)^{\top} (\bD_i)_j \bY^j\right] \le \frac{1}{n} D_1$. Using the Matrix Chernoff again, 
%$$ \Pr\left[ \sum_j (\bY^j)^{\top} (\bD_i)_j (\bY^j) \le (1+\delta) \frac{D_1}{n}\right] \le n e^{-\frac{\delta^2}{3} \frac{D_1}{n R}} \le n e^{-\delta^2 \log^2 n}$$ 
%Picking $\delta = \frac{1}{4}$, and union bounding over all $i$, with probability $1 - \frac{1}{\mbox{poly}}$, for all $i$,  
%$$ \sigma_{\max}\left(\bY^{\top} \bD_i \bY\right)  \le \frac{5}{4} \frac{D_1}{n}$$
%\Anote{Uses $\|W\|_{\infty} \le \frac{D_1}{10 \log^2 n}$, which is mild. }
%Furthermore, let 
%$$ \sigma^2 = \|\sum_k \mathbb{E}[(\bY^k (\bD_i)_k (\bY^k)^{\top})^2] \| \le  \sum_k \|\mathbb{E}[(\bY^k (\bD_i)_k (\bY^k)^{\top})^2]\| \le 100 \frac{\lambdau^2}{\mu^2}$$
%where the last inequality is again by our definition of $\bY$. 
%Applying Matrix Chernoff we get that
%$$\Pr[ \sum_k \bY^k (\bD_i)_k (\bY^k)^{\top} \ge t] \le n \exp(-t^2/(\sigma^2 + Rt/3)) \le n \exp(-\frac{\mu}{200} \frac{t^2}{\lambdau^2})$$  

%For a value $g > 0$, we call $j \in [n]$ ``good'' if $\| \bY^j   - \bV^j \|_2^2 \le g^2$. Denote the set of ``good'' $j$ as $\set{S}_g$, then we have:

%For every unit vector $a \in \Real^k$, 
%\begin{eqnarray*}
%a^{\top} \bY^{\top} \bD_i \bY a &=& \sum_{j \in [n]} (\bD_i)_j \langle a, \bY^j \rangle^2
%\\
%&=&\sum_{j} (\bD_i)_j \left(\langle a, \bV^j \rangle +  \langle a, \bY^j - \bV^j \rangle \right)^2
%\\
%&\ge& \frac{3}{4}\sum_{j} (\bD_i)_j \langle a, \bV^j \rangle^2 - 3 \sum_{j} (\bD_i)_j  \langle a, \bY^j - \bV^j \rangle^2 \quad ....\forall x, y \in \Real: (x + y)^2 \ge \frac{3}{4}x^2 - 3y^2 \\
%&\ge& \frac{3}{4}\sum_{j} (\bD_i)_j \langle a, \bV^j \rangle^2 - 3\sum_{j} (\bD_i)_j  (\|\bY^j\|^2 +\|\bV^j\|^2 - 2 \langle \bY^j, \bV^j \rangle) 
%\end{eqnarray*} 
%
%Consider picking $a$ at random. Then, with high probability ...  
%\begin{eqnarray*} 
%& & \frac{3}{4}\sum_{j} (\bD_i)_j \langle a, \bV^j \rangle^2 - 3 \sum_{j} (\bD_i)_j  \langle a, \bY^j - \bV^j \rangle^2 \\
%&\ge& \frac{3}{4}\sum_{j} (\bD_i)_j \langle a, \bV^j \rangle^2 - \frac{3}{n}\sum_{j} (\bD_i)_j  \|a\|^2 \|\bY^j - \bV^j\|^2 \\
%&=&\frac{3}{4}\sum_{j} (\bD_i)_j \langle a, \bV^j \rangle^2 - \frac{3}{n} \sum_{j} (\bD_i)_j  (\|\bY^j\|^2 +\|\bV^j\|^2 - 2 \langle \bY^j, \bV^j \rangle)
%\end{eqnarray*}
%
%By the assumptions on the model, 
%$$\sum_{j \in [n]} (\bD_i)_j \langle a, \bV^j \rangle^2 = a^T \bV^{\top} \bD_i \bV a \ge \sigma_{\min} (\bV^{\top} \bD_i \bV) \ge \lambdal $$
%
%On the other hand, since ... is picked at random ..., $\|\bY^j\|^2 \leq \frac{\mu k}{n}$ with probability .... Hence, with probability ..., 
%
%\begin{eqnarray*}
%& & \frac{3}{4} \lambdal - 3 \sum_{j} (\bD_i)_j  (\|\bY^j\|^2 +\|\bV^j\|^2 - 2 \langle \bY^j, \bV^j \rangle) \\
%&\ge& \frac{3}{4}\lambdal- 12 \sum_{j} (\bD_i)_j  \frac{\mu k}{n} \\
%&\ge& \frac{3}{4}\lambdal - 12 \frac{\lambdal^2 n}{k \lambdau \log n} 
%\end{eqnarray*} 

\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:alt_min_rand}]

%We show that the proof using SVD initialization can be easily modified to work with our random initialization as well, at the expense of ... 
Let $\bY$ be initialized using the random initialization algorithm \ref{alg:rinitial}. Consider applying the proof in Lemma \ref{lem:update_main}, with $\set{S}_1$ being modified to be  
$$\set{S}_1 = \left\{ i  \in [n]\left| \sigma_{\min} (\bY^{\top} \bD_i \bY) \le \frac{\lambdal}{4 \mu k} \right. \right\} $$ 
But with this modification, $\set{S}_1 = \emptyset$, with high probability. With this modification, the same calculation from Lemma \ref{lem:update_main} (which now doesn't need to use Lemma \ref{lem:sigma_min} at all) gives 
$$ \left\| \bbX - \bU \bSigma \bV^{\top} \bY \right \|_F^2 \leq \Delta_g \mu k $$
But following part (2) of the same Lemma, we get that if $\Delta_g \mu k < \frac{1}{8} \sigma_{\min}(M^{*})$, 
$$ \cds(\bU, \bX) \le \frac{2}{\sigma_{\min}(\bMg) - 2 \Delta_g \mu k } \Delta_g \mu k $$

So, in order to argue by induction in \ref{thm:alt_min} exactly as before, we only need to check that after the update step for $\bX$, $\cds(\bU, \bX)$ is small enough to apply Lemma \ref{lem:update_main}:  
$$\cds(\bU, \bX) \le \frac{2}{\sigma_{\min}(\bMg) - 2 \Delta_g \mu k } \Delta_g \mu k \le \sqrt{\min\{\frac{1}{2}, \frac{\lambdal^2 n}{384 \mu k^2 \dmax} \}} $$ 

Noticing that $\Delta_g$ has a quadratic dependency on $\gamma$, we see that if 
\begin{align*}
\gamma  = O\left( \min\left\{ \sqrt{\frac{n}{D_1}}\frac{\lambdal \sigma_{\min}(\bMg) }{ \mu^{2} k^{5/2}} , 
\frac{\lambdal \sigma^{3/2}_{\min}(\bMg)}{\mu^{3/2} k^{5/2}}    \right\} \right),
\end{align*}
the inequality is indeed satisfied. 

With that, the theorem statement follows. 

\end{proof} 
